Improved Dynamic Algorithms for Longest Increasing Subsequence

We study dynamic algorithms for the longest increasing subsequence (\textsf{LIS}) problem. A dynamic \textsf{LIS} algorithm maintains a sequence subject to operations of the following form arriving one by one: (i) insert an element, (ii) delete an element, or (iii) substitute an element for another. After performing each operation, the algorithm must report the length of the longest increasing subsequence of the current sequence. Our main contribution is the first exact dynamic \textsf{LIS} algorithm with sublinear update time. More precisely, we present a randomized algorithm that performs each operation in time $\tilde O(n^{2/3})$ and after each update, reports the answer to the \textsf{LIS} problem correctly with high probability. We use several novel techniques and observations for this algorithm that may find their applications in future work. In the second part of the paper, we study approximate dynamic \textsf{LIS} algorithms, which are allowed to underestimate the solution size within a bounded multiplicative factor. In this setting, we give a deterministic algorithm with update time $O(n^{o(1)})$ and approximation factor $1-o(1)$. This result substantially improves upon the previous work of Mitzenmacher and Seddighin (STOC'20) that presents an $\Omega(\epsilon ^{O(1/\epsilon)})$-approximation algorithm with update time $\tilde O(n^\epsilon)$ for any constant $\epsilon > 0$.

==> src/extended-grid-packing.tex <==
\section{Beyond Grid Packing}\label{sec:dynamic}
In this section, we bring an introduction to the grid packing technique and discuss how we extend the idea to improve the approximation factor of our dynamic algorithm for \textsf{LIS}. We first give a background of grid packing in Section~\ref{sec:previous} and then explain our extension. We illustrate how the extended grid packing technique can be used to design improved algorithms for \textsf{LIS} in Section~\ref{sec:dynamic}.
\subsection{Background: Grid Packing}\label{sec:previous}



==> tables/dynamic.tex <==
\begin{table}[!htbp]
	\centering
	\begin{tabular}{|l|c|c|c|c|c|c|c|}
		\hline
		algorithm & $m$ & $f(n)$ & $g(n)$ & $h_1(n)$ & $h_2(n)$ &$h(n)$ & $f(n)/g(n) + h(n)$\\
		\hline
$\mathcal{A}_{1}$ & $n^{4/7}$ & $n^{19/7}$ & $n^{3/7}$ & $n^{15/7}$ & $n^{16/7}$ & $n^{16/7}$ & $n^{16/7}$\\
\hline
$\mathcal{A}_{2}$ & $n^{4/11}$ & $n^{20/11}$ & $n^{7/11}$ & $n^{16/11}$ & $n^{16/11}$ & $n^{16/11}$ & $n^{16/11}$\\
\hline
$\mathcal{A}_{3}$ & $n^{4/15}$ & $n^{4/3}$ & $n^{11/15}$ & $n^{16/15}$ & $n^{16/15}$ & $n^{16/15}$ & $n^{16/15}$\\
\hline
$\mathcal{A}_{4}$ & $n^{4/19}$ & $n^{20/19}$ & $n^{15/19}$ & $n^{16/19}$ & $n^{16/19}$ & $n^{16/19}$ & $n^{16/19}$\\
\hline
$\mathcal{A}_{5}$ & $n^{4/23}$ & $n^{20/23}$ & $n^{19/23}$ & $n^{16/23}$ & $n^{16/23}$ & $n^{16/23}$ & $n^{16/23}$\\
\hline
$\mathcal{A}_{6}$ & $n^{4/27}$ & $n^{20/27}$ & $n^{23/27}$ & $n^{16/27}$ & $n^{16/27}$ & $n^{16/27}$ & $n^{16/27}$\\
\hline
$\mathcal{A}_{7}$ & $n^{4/31}$ & $n^{20/31}$ & $n^{27/31}$ & $n^{16/31}$ & $n^{16/31}$ & $n^{16/31}$ & $n^{16/31}$\\
\hline
$\mathcal{A}_{8}$ & $n^{4/35}$ & $n^{4/7}$ & $n^{31/35}$ & $n^{16/35}$ & $n^{16/35}$ & $n^{16/35}$ & $n^{16/35}$\\
\hline
$\mathcal{A}_{9}$ & $n^{4/39}$ & $n^{20/39}$ & $n^{35/39}$ & $n^{16/39}$ & $n^{16/39}$ & $n^{16/39}$ & $n^{16/39}$\\
\hline
$\mathcal{A}_{10}$ & $n^{4/43}$ & $n^{20/43}$ & $n^{39/43}$ & $n^{16/43}$ & $n^{16/43}$ & $n^{16/43}$ & $n^{16/43}$\\
\hline
$\mathcal{A}_{11}$ & $n^{4/47}$ & $n^{20/47}$ & $n^{43/47}$ & $n^{16/47}$ & $n^{16/47}$ & $n^{16/47}$ & $n^{16/47}$\\
\hline

	
	\end{tabular}
	\caption{$q_i$ is the exponent of $n$ in the preprocessing time of Algorithm $\mathcal{A}_i$.}\label{table:static}
\end{table}
